A Calculus of Looping Sequences with Local Rules

In this paper we present a variant of the Calculus of Looping Sequences (CLS for short) with global and local rewrite rules. While global rules, as in CLS, are applied anywhere in a given term, local rules can only be applied in the compartment on which they are defined. Local rules are dynamic: they can be added, moved and erased. We enrich the new calculus with a parallel semantics where a reduction step is lead by any number of global and local rules that could be performed in parallel. A type system is developed to enforce the property that a compartment must contain only local rules with specific features. As a running example we model some interactions happening in a cell starting from its nucleus and moving towards its mitochondria.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{E. Kashefi, J. Krivine, F. van Raamsdonk (Eds.) \\
DCM 2011\\
EPTCS 88, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.88.4}{10.4204/EPTCS.88.4}}

